Steering Feedback in Dynamic Driving Simulators: The Influence of Steering Wheel Vibration and Vehicle Motion Frequency

The validity of the subjective evaluation of steering feedback in driving simulators is crucial for modern vehicle development. Although there are established objective steering characteristics for the assessment of both stationary and dynamic feedback behaviour, factors such as steering wheel vibrations and vehicle body motion, particularly in high-frequency ranges, present challenges in simulator fidelity. This work investigates the influence of steering wheel vibration and vehicle body motion frequency content on the subjective evaluation of steering feedback during closed-loop driving in a dynamic driving simulator. A controlled subject study with 30 participants consisting of a back-to-back comparison of a reference vehicle with an electrical power steering system and three variants of its virtual representation on a dynamic driving simulator was performed. Subjective evaluation focused on the representation of road feedback in comparison to the reference vehicle. The statistical analysis of subjective results show that there is a significant influence of the frequency content of both steering wheel torque and vehicle motion on the subjective evaluation of steering feedback in a dynamic driving simulator. The results suggest an influence of frequency content on the subjective evaluation quality of steering feedback characteristics that are not associated with the dynamic feedback behaviour in the context of established performance indicators.

==> fig_Box_RoadContactAllVars.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{Box_RoadContactAllVars.pdf}
\caption{Z-transformed ratings of Road contact across all variants}
\label{fig_Box_RoadContactAllVars}
\end{figure}


==> fig_Spider_RoadContactAllVars.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=2.5in]{Spider_RoadContactVarAllVars39.pdf}
    \caption{Absolute value of Road contact ratings (higher is better)
    % TODO: Add legend
    }
    \label{fig_Spider_RoadContactAllVars}
    \end{figure}
    
